Tags2Parts: Discovering Semantic Regions from Shape Tags

We propose a novel method for discovering shape regions that strongly correlate with user-prescribed tags. For example, given a collection of chairs tagged as either "has armrest" or "lacks armrest", our system correctly highlights the armrest regions as the main distinctive parts between the two chair types. To obtain point-wise predictions from shape-wise tags we develop a novel neural network architecture that is trained with tag classification loss, but is designed to rely on segmentation to predict the tag. Our network is inspired by U-Net, but we replicate shallow U structures several times with new skip connections and pooling layers, and call the resulting architecture "WU-Net". We test our method on segmentation benchmarks and show that even with weak supervision of whole shape tags, our method can infer meaningful semantic regions, without ever observing shape segmentations. Further, once trained, the model can process shapes for which the tag is entirely unknown. As a bonus, our architecture is directly operational under full supervision and performs strongly on standard benchmarks. We validate our method through experiments with many variant architectures and prior baselines, and demonstrate several applications.

==> acks.tex <==
\section*{Acknowledgements}


==> apps.tex <==
\section{Applications}

In this section, we demonstrate the wide utility of our method by presenting a few potential applications. We believe that our approach can benefit anyone who needs to quickly identify and discover semantic parts that characterize large classes of shapes, without having the resources to gather fine-grained part annotations. Hence, this list is hardly exhaustive.

\begin{figure}[b!]
  \includegraphics[width=1.0\linewidth]{figures/search.jpg}
  \caption{Each row shows the top 3 shapes with similar armrests, detected by \wunet, retrieved for the query in the first column.}
  \label{fig:search}
\end{figure}

\paragraph{Part-sensitive shape search.} 3D shape search has been extensively studied~\cite{Tangelder2007}. Our approach enables  {\em part-sensitive search}, where shapes with a particular part similar to a given shape are sought, to be implemented cheaply and quickly, since crowdsourced shape tags can be easily obtained (cf. the abundance of image tags in Flickr, but the relative paucity of pixel-level image segmentations). Further since \wunet has very high pure classification performance, it can directly infer tags on unseen shapes as well, allowing the dataset to be rapidly expanded and segmented.

We show a prototype interface in Figure \ref{fig:search}. A query shape and a tag are provided. Shapes in the dataset preprocessed by \wunet for this tag are retrieved based on similarity in the salient region (our simple implementation uses weighted average distance between the salient voxels, after the centroids of the salient regions are aligned).

\begin{figure}[t!]
  \includegraphics[width=1.0\linewidth]{figures/embedding.jpg}
  \caption{A t-SNE embedding of chairs organized by similarity of the ``armrest'' regions detected by \wunet. Below, we show several zoomed-in regions of the image. The larger icons on top represent diverse representatives of the collection that can be obtained from this similarity metric.}
  \label{fig:embedding}
\end{figure}

\paragraph{Fine-grained exploration of a shape dataset.} The part-sensitive similarity metric computed for the search application can also be used to organize the complete dataset. In Figure \ref{fig:embedding} we show a t-SNE embedding of our chair dataset based on similarity of the detected ``armrest'' region. Note that the embedding places shapes with broadly similar arms together even if the rest of shape is quite different. A person can quickly get a visual overview of the variation of armrests in the dataset from this embedding, and perhaps discover new types of armrests.

In the same embedding, we highlight representative shapes which have very different armrests. This type of information, which is very valuable in gauging the variance and range of the dataset, is a direct byproduct of our inferred part annotations.

\paragraph{Thumbnail creation.} When large numbers of shapes need to be presented for rapid browsing, it is helpful to have access to thumbnail representations which nevertheless capture the salient aspects of the shapes~\cite{Shilane2007}. The \wunet output directly enables such an application where the generated icons capture semantic parts. In Figure \ref{fig:icon}, we show examples of different thumbnails generated for the same shape that highlight different semantic aspects of the shape.

\begin{figure}[t!]
  \includegraphics[width=1.0\linewidth]{figures/icon.jpg}
  \caption{Different thumbnails of the same shapes (first column) created to highlight detected ``armrest'' (second column) and ``back'' (third column) regions.}
  \label{fig:icon}
\end{figure}

